To CoT or not to CoT? Chain-of-thought helps mainly on math and symbolic reasoning

Chain-of-thought (CoT) via prompting is the de facto method for eliciting reasoning capabilities from large language models (LLMs). But for what kinds of tasks is this extra ``thinking'' really helpful? To analyze this, we conducted a quantitative meta-analysis covering over 100 papers using CoT and ran our own evaluations of 20 datasets across 14 models. Our results show that CoT gives strong performance benefits primarily on tasks involving math or logic, with much smaller gains on other types of tasks. On MMLU, directly generating the answer without CoT leads to almost identical accuracy as CoT unless the question or model's response contains an equals sign, indicating symbolic operations and reasoning. Following this finding, we analyze the behavior of CoT on these problems by separating planning and execution and comparing against tool-augmented LLMs. Much of CoT's gain comes from improving symbolic execution, but it underperforms relative to using a symbolic solver. Our results indicate that CoT can be applied selectively, maintaining performance while saving inference costs. Furthermore, they suggest a need to move beyond prompt-based CoT to new paradigms that better leverage intermediate computation across the whole range of LLM applications.

==> images/fs_cot_vs_direct/fs_cot_vs_direct_figure.tex <==
\begin{figure}[t!]
    \centering

    \includegraphics[width=1.0\linewidth, trim=0mm 30mm 0mm 30mm]{images/fs_cot_vs_direct/fs_non_symbolic.png}
    \vspace{10mm} % Add vertical space here

    \includegraphics[width=1.0\linewidth, trim=0mm 30mm 0mm 30mm]{images/fs_cot_vs_direct/fs_semi_symbolic.png}
    \vspace{10mm} % Add vertical space here

    \includegraphics[width=1.0\linewidth, trim=0mm 30mm 0mm 30mm]{images/fs_cot_vs_direct/fs_symbolic.png}
    \vspace{5mm} % Add vertical space here

    \caption{ 
       Performance of Few-Shot Direct (Blue) and Few-Shot CoT (Orange) across the three classes of datasets: Non-symbolic, Semi-symbolic, and Symbolic.  Notice that the majority of semi-symbolic and symbolic datasets will benefit from CoT across all models despite there being applicable reasoning that can be used to benefit Non-symbolic datasets as well.
    }
    \label{fig:fs_exp_0_plot}
    
    % \vspace*{-.15in}

\end{figure}


==> tables/bbh_table.tex <==
\begin{table}
\centering
\begin{scriptsize}  % Reduced font size
\setlength{\tabcolsep}{4pt}  % Adjust column separation
\resizebox{\textwidth}{!}{  % Resize to fit within text width
\begin{tabular}{l|c|c|c|c|c|c}
\toprule
 subject                                 &   \rotatebox{45}{Meta-Llama 2 7b} &   \rotatebox{45}{Mistral 7b} &   \rotatebox{45}{Meta-Llama 3.1 8b} &   \rotatebox{45}{Meta-Llama 3.1 70b} &   \rotatebox{45}{Gemma 2 9b} &   \rotatebox{45}{Phi-3 Small 8k} \\
\midrule
 hyperbaton                              &              10.4 &         -4.8 &                 8.8 &                -20.8 &          2.8 &             -8.8 \\
 logical\_deduction\_three\_objects         &              -4.8 &         -8.4 &                19.6 &                -10.4 &          0.4 &              5.6 \\
tracking\_shuffled\_objects\_seven\_objects &               6   &         -0.4 &                40   &                 12.4 &         66   &             40.8 \\
 date\_understanding                      &               4.8 &          3.2 &                23.6 &                 73.2 &         62   &              8.4 \\
ruin\_names                              &               7.7 &          3.2 &                -4.4 &                 -3.2 &         -2.4 &              0.8 \\
dyck\_languages                          &             -14.8 &         -9.2 &               -12   &                  0.4 &          7.6 &             -2.4 \\
temporal\_sequences                      &              21.2 &          6.4 &                16   &                 46.8 &         78.4 &             -1.2 \\
boolean\_expressions                     &               1.2 &        -22   &                 9.6 &                -10.4 &          9.2 &              0   \\
multistep\_arithmetic\_two                &               3.2 &          1.6 &                73.2 &                 26.4 &          5.6 &             81.2 \\
reasoning\_about\_colored\_objects         &              -2   &         -0.4 &                20.8 &                 -2   &         10.8 &             14   \\
tracking\_shuffled\_objects\_five\_objects  &              11.2 &         -4.8 &                39.2 &                  9.6 &         63.6 &             47.6 \\
penguins\_in\_a\_table                     &              -2.1 &         13.7 &                36.3 &                 47.3 &         49.3 &             18.5 \\
 navigate                                &              14.8 &         -2.8 &                28   &                  0.4 &          2   &             -8.4 \\
geometric\_shapes                        &              -4   &         -3.6 &                12.8 &                  4   &         19.2 &             -2   \\
snarks                                  &             -12.4 &         -4.5 &                12.9 &                 -8.4 &          3.4 &            -10.7 \\
word\_sorting                            &               0   &          0   &                 0.4 &                  4   &          2   &             -1.6 \\
movie\_recommendation                    &             -18.1 &        -21.3 &                -2   &                -17.7 &         -6.8 &            -16.1 \\
object\_counting                         &               7.6 &         -7.2 &                19.6 &                  8   &          5.6 &              6.4 \\
web\_of\_lies                             &               5.6 &          0.4 &                38   &                 28   &         42.8 &             11.6 \\
logical\_deduction\_seven\_objects         &               7.2 &          0.4 &                 0.4 &                  2   &         -3.2 &             -5.2 \\
formal\_fallacies                        &             -12.4 &          1.2 &                 1.6 &                -27.6 &         -6.8 &             -4.8 \\
tracking\_shuffled\_objects\_three\_objects &             -11.2 &          4   &                48.4 &                  2.8 &         50.8 &             37.2 \\
logical\_deduction\_five\_objects          &               6.8 &          6   &                15.6 &                 -1.2 &          8   &             -0.4 \\
disambiguation\_qa                       &             -12.4 &         -6   &                 0   &                -10   &         -5.6 &             -3.6 \\
salient\_translation\_error\_detection     &              30.4 &         -1.2 &                 4   &                -12.8 &         -8   &             -6.8 \\
 causal\_judgement                        &              -0.5 &          2.7 &                -0.5 &                -33.2 &        -12.3 &            -16   \\
\bottomrule
\end{tabular}}
\end{scriptsize}
\label{tab:bbh_results}
\caption{Results of multiple models on the BigBench-Hard dataset reporting the CoT - Direct delta for each task.}
\end{table}

==> tables/exp_2_causal_prefix.tex <==
\begin{table}
\small
\centering

%\renewcommand{\tabcolsep}{0.9mm}
\begin{tabular}{c|cccc|cccc}
\toprule 
& \multicolumn{4}{c}{Llama 3 8b} & \multicolumn{4}{c}{Llama 3 70b} \\\midrule
  & Acc Change & Px Acc $\triangle$ & Shift Change & Px Shift $\triangle$ & Acc Change & Px Acc $\triangle$ & Shift Change & Px Shift $\triangle$ \\\midrule
MM-MuSR & .0 & .05 & .06 & .18 & .0 & .0 & .02 & .08 \\
StrategyQA & .0 & .0 & .04 & .04 & .0 & .0 & .02 & .0 \\
CSQA & -.04 & .08 & -.02 & .13 & .0 & .0 & .03 & .02 \\
Winogrande & -.02 & .04 & -.02 & .08 & -.02 & .0 & .0 & .02 \\

\bottomrule
\end{tabular}
\label{tab:exp_2_causal_analysis}
\caption{MM-MuSR is the murder mystery slice of the MuSR dataset.  Acc Change is the difference in accuracy from using the original prefix vs. the new prefix averaged across all the semantically equivalent prefix pairs on which we ran the dataset. Px Acc $\triangle$ is the difference in performance between the pairs of prefixes averaged. Shift Change is the measure of change in the Shift metric from the previous experiment using the new prefix. px Shift $\triangle$ is the difference in the shift metric between the pairs of prefixes averaged. We see that using different prefixes with the same reasoning as the original prefix does fully explain the performance variance between the prefixes. This means that the prefixes selected in experiment 1 elicit different reasoning from the language model, giving different performances despite the prefixes being equivalent semantically. Furthermore, we can be sure that the performance differences are not entirely attributed to the tokens of the prefix themselves, instead it's what the prefixes lead to in the generation. \zayne{double check this. Lost some confidence in this experiment because I think CoTs can say the answer before giving the parseable answer text, which might trivialize the experiment here (we'd need a better way of catching and stripping out the answer).  Also, I want to make sure the equivalent prefixes lead to different performance on the dataset but same performances here.}}
% \vspace{-.25in}
\end{table}




==> tables/icl_experiment.tex <==
\begin{table}
\centering
\begin{scriptsize}  % Reduced font size
\setlength{\tabcolsep}{4pt}  % Adjust column separation
\resizebox{\textwidth}{!}{  % Resize to fit within text width
\begin{tabular}{ll|cc}
\toprule
 Dataset                 & Type      &   Zero-shot CoT - Direct Delta &   Few-shot CoT - Direct Delta \\
\midrule
 CommonsenseQA           & Non-Symbolic  &                         -0.018 &                         \phantom{-}0.008 \\
 StrategyQA              & Non-Symbolic  &                          \phantom{-}0.018 &                         \phantom{-}0.035 \\
 \midrule
 AGIEval LSAT LR         & Semi-Symbolic &                         -0.015 &                        -0.01\phantom{0}  \\
 AGIEval LSAT AR         & Semi-Symbolic &                          \phantom{-}0.012 &                         \phantom{-}0.006 \\
 AGIEval LSAT RC         & Semi-Symbolic &                         -0.014 &                        -0.042 \\
 Murder Mysteries MuSR   & Semi-Symbolic &                          \phantom{-}0.091 &                         \phantom{-}0.077 \\
 Team Allocations MuSR   & Semi-Symbolic &                         -0.049 &                         \phantom{-}0.068 \\
 Object Placements MuSR  & Semi-Symbolic &                          \phantom{-}0.069 &                         \phantom{-}0.134 \\
 MMLU                    & Semi-Symbolic &                          \phantom{-}0.034 &                         \phantom{-}0.03\phantom{0}   \\
 MMLU Pro                & Semi-Symbolic &                          \phantom{-}0.093 &                         \phantom{-}0.096 \\
 GPQA                    & Semi-Symbolic &                          \phantom{-}0.019 &                        -0.001 \\
 GSM8K                   & Semi-Symbolic &                          \phantom{-}0.593 &                         \phantom{-}0.545 \\
 \midrule
 ContextHub Deductive L1 & Symbolic      &                          \phantom{-}0.127 &                         \phantom{-}0.2\phantom{0}\phantom{0}    \\
 ContextHub Deductive L2 & Symbolic      &                          \phantom{-}0.118 &                         \phantom{-}0.217 \\
 ContextHub Abductive L1 & Symbolic      &                          \phantom{-}0.118 &                         \phantom{-}0.033 \\
 ContextHub Abductive L2 & Symbolic      &                          \phantom{-}0.075 &                         \phantom{-}0.065 \\
 MATH                    & Symbolic      &                          \phantom{-}0.286 &                         \phantom{-}0.277 \\
\bottomrule
\end{tabular}}
\end{scriptsize}
\label{tab:icl_experiment}
\caption{Showing the effects of Few-shot examples when prompting with Chain of Thought.  Here, we report the average Chain of thought performance minus the Direct performance across models per dataset. The only dataset to have a large performance boost where Chain of Thought starts to actually help is Team Allocation MuSR.  We believe this may be an artifact of the specific dataset and prompt rather than an exception to the rule. For all other datasets, CoT in the few shot setting does not change when CoT helps, though it can change the magnitude. }
\end{table}

==> tables/log_model_performances.tex <==
\begin{table}
\small
\begin{tabular}{lrrrrrrrrrr}
\toprule
 dataset                 &   \text{=} &   CoT Helps &   Direct &   CoT &   Log &   Total Toks &   Saved Toks &  \# CoTs &   \# Directs &   Total \\
\midrule
 CommonsenseQA           &      99 &              94 &           77 &        75 &        77 &              651 &          633 &             12 &              1209 &    1221 \\
 StrategyQA              &      99 &              92 &           70 &        71 &        70 &             1613 &         1503 &             27 &              2794 &    2821 \\
 SiQA                    &     100 &              92 &           59 &        60 &        59 &              944 &          931 &              0 &              1954 &    1954 \\
 PiQA                    &      98 &              92 &           83 &        84 &        83 &              903 &          882 &             30 &              1808 &    1838 \\
 Winogrande              &     100 &              91 &           69 &        71 &        69 &              469 &          462 &              1 &              1266 &    1267 \\
 Arc Easy                &      94 &              92 &           91 &        92 &        91 &              382 &          357 &             34 &               536 &     570 \\
 Arc Challenge           &      94 &              88 &           82 &        85 &        83 &              210 &          195 &             21 &               278 &     299 \\
 AGIEval LSAT LR         &      98 &              89 &           59 &        58 &        59 &              603 &          579 &              9 &               501 &     510 \\
 AGIEval LSAT AR         &      59 &              55 &           23 &        24 &        23 &              302 &          182 &             93 &               137 &     230 \\
 AGIEval LSAT RC         &     100 &              92 &           68 &        67 &        68 &              302 &          295 &              0 &               269 &     269 \\
 ContextHub Deductive L1 &      95 &              80 &           39 &        52 &        40 &              294 &          270 &             29 &               571 &     600 \\
 ContextHub Deductive L2 &      93 &              80 &           37 &        49 &        38 &             1516 &         1365 &            158 &              1955 &    2112 \\
 ContextHub Abductive L1 &      73 &              66 &           40 &        52 &        44 &              211 &          153 &             95 &               265 &     360 \\
 ContextHub Abductive L2 &      85 &              75 &           37 &        44 &        39 &             1776 &         1502 &            306 &              1807 &    2112 \\
 Murder Mysteries MuSR   &     100 &              84 &           60 &        71 &        60 &              318 &          316 &              0 &               250 &     250 \\
 Team Allocations MuSR   &     100 &              85 &           54 &        57 &        54 &              427 &          421 &              0 &               250 &     250 \\
 Object Placements MuSR  &     100 &              77 &           48 &        59 &        48 &              191 &          189 &              0 &               236 &     236 \\
 MMLU                    &      96 &              84 &           68 &        72 &        70 &             7479 &         6317 &           1765 &             12277 &   14042 \\
 MMLU Pro                &      93 &              62 &           39 &        49 &        47 &             9304 &         4882 &           5370 &              6662 &   12032 \\
 MATH                    &      89 &              34 &           16 &        44 &        42 &             4594 &          251 &           4651 &               347 &    4998 \\
 GSM8K                   &      78 &              57 &           18 &        79 &        65 &              880 &          179 &           1030 &               289 &    1319 \\
\bottomrule
\end{tabular}
\caption{
Token counts are shown in units of 1000 to fit the data within the table.
}
\end{table}

==> tables/mmlu_aggregate.tex <==
\begin{table}
\small
\centering
\begin{tabular}{l|rrr|rrr}

\toprule
 &  \multicolumn{3}{c}{MMLU} & \multicolumn{3}{c}{MMLU Pro} \\
 Model   &   Direct &   CoT &  Delta &   Direct &   CoT &   Delta \\
\midrule
 3 8b    &              0.61 &           0.64 &         0.03 &                  0.32 &               0.39 &             0.06 \\
 3 70b   &              0.77 &           0.79  &         0.02 &                  0.47 &               0.59 &             0.12 \\
 3.1 8b  &              0.67 &           0.71 &         0.04 &                  0.38 &               0.47 &             0.09 \\
 3.1 70b &              0.81 &           0.85 &         0.04 &                  0.52 &               0.66 &             0.14 \\
\bottomrule

\end{tabular}
\caption{Accuracies for models on MMLU and MMLU Pro in two different settings.  ``Direct'' refers to prompting the language model zero-shot without asking for a chain of though. ``CoT'' refers to \zayne{ cite kojima } prompting the language model zero-shot asking for a chain of thought before the answer.  Notice that CoT hardly helps on MMLU while significantly helps on MMLU Pro.}
\label{tab:mmlu_aggregate}
\end{table}

==> tables/mmlu_clustering_efficiency_performance.tex <==
\begin{table}
\small

\begin{tabular}{lrrrrrrrrrrrr}
\toprule
&\multicolumn{3}{c}{MMLU} &\multicolumn{3}{c}{MMLU Pro} &\multicolumn{3}{c}{MATH} &\multicolumn{3}{c}{GSM8k} \\

 Model       &   D &   R &     S &   D &   R &     S &   D &   R &    S &   D &   R &    S \\
\midrule
 G2 9b       &   0 &  87 &  5.9  &   2 &  77 &  2.9  &   2 &  94 & 0.19 &  13 &  79 & 0.11 \\
 GPT-4o mini &   2 &  69 &  5.05 &   3 &  85 &  6.55 &   3 &  94 & 0.3  &  14 &  78 & 0.28 \\
 L 3.1 70b   &  -0 & 105 &  7.42 &   0 &  96 &  3.91 &   3 &  94 & 0.32 &  16 &  76 & 0.19 \\
 L2 7b       &   4 &  11 & 10.29 &  -1 & -69 & 12.54 &  -0 &  88 & 0.1  &   5 &  81 & 0.15 \\
 L3.1 8b     &   2 &  60 &  8.1  &   2 &  76 &  5.09 &   2 &  94 & 0.32 &  18 &  78 & 0.24 \\
 M 7b        &   3 &  32 &  5.96 &   1 &  48 &  1.93 &   0 &  96 & 0.29 &  10 &  79 & 0.17 \\
 P3-small    &   1 &  61 &  3.02 &   2 &  83 &  2.23 &   2 &  93 & 0.18 &  16 &  79 & 0.13 \\
 Q 72b       &   1 &  70 &  4.8  &   3 &  84 &  3.91 &   2 &  94 & 0.32 &  13 &  79 & 0.16 \\
\bottomrule
\end{tabular}
\label{tab:classifier_recovery_performances}
\caption{Table reporting the delta, ``D'', between CoT performance and Selective CoT using our classifier $g'$ as the method for deciding when to use CoT over Direct prompts.  ``R'' shows the percentage of performance recovered over using Direct prompts only when compared to CoT. ``S'' shows the number of tokens saved in the millions.  We can see that for nearly all models and tasks we recover at least 75\% of the original performance over direct while saving millions of tokens.  For MMLU not only can we fully recover the performance on Llama 3.1 70B but actually improve on MMLU over CoT and recover nearly all of the MMLU Pro performance (96\%) while saving 7 and 4 million tokens respectively.}
\end{table}



==> tables/mmlu_slices.tex <==
\begin{table}[ht]
\centering
\begin{scriptsize}  % Reduced font size
\setlength{\tabcolsep}{4pt}  % Adjust column separation
\resizebox{\textwidth}{!}{  % Resize to fit within text width
\begin{tabular}{lrrrr}    
\toprule
\multicolumn{5}{c}{CoT - Direct Performance of Meta-Llama 3.1 8b on MMLU Categories}\\
\midrule
Subject                             &   Direct Acc (\%) &   CoT Acc (\%) &   Error Reduction (\%) &    N \\
\midrule
 moral\_scenarios                     &               58 &            63 &                    12 &  895 \\
 college\_computer\_science            &               50 &            58 &                    16 &  100 \\
 high\_school\_macroeconomics          &               67 &            74 &                    23 &  390 \\
 business\_ethics                     &               63 &            73 &                    27 &  100 \\
 college\_mathematics                 &               34 &            49 &                    23 &  100 \\
 professional\_law                    &               50 &            52 &                     4 & 1534 \\
 marketing                           &               88 &            90 &                    11 &  234 \\
 miscellaneous                       &               84 &            90 &                    37 &  783 \\
 college\_medicine                    &               69 &            78 &                    28 &  173 \\
 high\_school\_biology                 &               81 &            82 &                     7 &  310 \\
 high\_school\_statistics              &               58 &            64 &                    14 &  216 \\
 high\_school\_psychology              &               87 &            89 &                    15 &  545 \\
 high\_school\_microeconomics          &               76 &            79 &                     9 &  238 \\
 professional\_psychology             &               71 &            73 &                     5 &  612 \\
 sociology                           &               79 &            81 &                     7 &  201 \\
 prehistory                          &               75 &            73 &                    -9 &  324 \\
 international\_law                   &               79 &            79 &                     4 &  121 \\
 security\_studies                    &               77 &            74 &                   -12 &  245 \\
 electrical\_engineering              &               69 &            69 &                     0 &  145 \\
 management                          &               83 &            85 &                    12 &  103 \\
 human\_sexuality                     &               75 &            82 &                    27 &  131 \\
 logical\_fallacies                   &               73 &            77 &                    14 &  163 \\
 econometrics                        &               55 &            57 &                     4 &  114 \\
 nutrition                           &               77 &            77 &                     3 &  306 \\
 human\_aging                         &               67 &            70 &                    10 &  223 \\
 medical\_genetics                    &               82 &            82 &                     0 &  100 \\
 high\_school\_chemistry               &               63 &            71 &                    22 &  203 \\
 moral\_disputes                      &               70 &            68 &                    -7 &  346 \\
 us\_foreign\_policy                   &               86 &            86 &                     0 &  100 \\
 philosophy                          &               70 &            71 &                     2 &  311 \\
 global\_facts                        &               35 &            52 &                    26 &  100 \\
 astronomy                           &               70 &            78 &                    24 &  152 \\
 virology                            &               53 &            55 &                     4 &  166 \\
 college\_biology                     &               83 &            85 &                     8 &  144 \\
 high\_school\_geography               &               83 &            85 &                     9 &  198 \\
 professional\_medicine               &               79 &            80 &                     4 &  272 \\
 elementary\_mathematics              &               47 &            88 &                    78 &  378 \\
 high\_school\_physics                 &               44 &            58 &                    24 &  151 \\
 high\_school\_mathematics             &               40 &            71 &                    53 &  270 \\
 anatomy                             &               70 &            76 &                    22 &  135 \\
 high\_school\_european\_history        &               77 &            75 &                   -11 &  165 \\
 computer\_security                   &               77 &            76 &                    -4 &  100 \\
 high\_school\_government\_and\_politics &               89 &            90 &                    10 &  193 \\
 world\_religions                     &               83 &            84 &                     3 &  171 \\
 clinical\_knowledge                  &               76 &            79 &                    11 &  265 \\
 abstract\_algebra                    &               33 &            46 &                    19 &  100 \\
 high\_school\_computer\_science        &               72 &            82 &                    36 &  100 \\
 conceptual\_physics                  &               62 &            73 &                    29 &  235 \\
 professional\_accounting             &               50 &            59 &                    18 &  282 \\
 formal\_logic                        &               50 &            59 &                    17 &  126 \\
 high\_school\_world\_history           &               85 &            86 &                     3 &  237 \\
 machine\_learning                    &               54 &            56 &                     6 &  112 \\
 high\_school\_us\_history              &               85 &            87 &                    10 &  204 \\
 jurisprudence                       &               72 &            70 &                    -7 &  108 \\
 college\_physics                     &               45 &            64 &                    34 &  102 \\
 college\_chemistry                   &               57 &            55 &                    -5 &  100 \\
 public\_relations                    &               70 &            69 &                    -3 &  110 \\
\bottomrule
\end{tabular}}
\end{scriptsize}
\end{table}

\begin{table}[ht]
\centering
\begin{scriptsize}  % Reduced font size
\setlength{\tabcolsep}{4pt}  % Adjust column separation
%\resizebox{\textwidth}{!}{  % Resize to fit within text width
\begin{tabular}{lrrrr}    
\toprule
\multicolumn{5}{c}{CoT - Direct Performance of Meta-Llama 3.1 8b on MMLU Pro Categories}\\
\midrule
Subject          &   Direct Acc (\%) &   CoT Acc (\%) &   Error Reduction (\%) &    N \\
\midrule
 engineering      &               36 &            25 &                   -17 &  969 \\
 health           &               53 &            57 &                     9 &  818 \\
 computer science &               40 &            50 &                    17 &  410 \\
 biology          &               59 &            59 &                    -1 &  717 \\
 psychology       &               60 &            62 &                     6 &  798 \\
 math             &               24 &            45 &                    28 & 1350 \\
 business         &               29 &            46 &                    23 &  789 \\
 economics        &               52 &            56 &                     9 &  844 \\
 chemistry        &               27 &            37 &                    14 & 1132 \\
 law              &               30 &            29 &                    -1 & 1101 \\
 physics          &               28 &            41 &                    19 & 1299 \\
 other            &               41 &            51 &                    16 &  924 \\
 history          &               44 &            44 &                     1 &  381 \\
 philosophy       &               39 &            42 &                     4 &  499 \\
\bottomrule
\end{tabular}
\end{scriptsize}
\end{table}

\begin{table}[ht]
\centering
\begin{scriptsize}  % Reduced font size
\setlength{\tabcolsep}{4pt}  % Adjust column separation
\resizebox{\textwidth}{!}{  % Resize to fit within text width
\begin{tabular}{lrrrr}    
\toprule
\multicolumn{5}{c}{CoT - Direct Performance of Meta-Llama 3.1 70b on MMLU Categories}\\
\midrule
Subject                             &   Direct Acc (\%) &   CoT Acc (\%) &   Error Reduction (\%) &    N \\
\midrule
 moral\_scenarios                     &               89 &            89 &                     0 &  895 \\
 college\_computer\_science            &               68 &            80 &                    38 &  100 \\
 high\_school\_macroeconomics          &               88 &            91 &                    29 &  390 \\
 business\_ethics                     &               82 &            80 &                   -11 &  100 \\
 college\_mathematics                 &               62 &            73 &                    29 &  100 \\
 professional\_law                    &               70 &            64 &                   -17 & 1534 \\
 marketing                           &               94 &            94 &                    -7 &  234 \\
 miscellaneous                       &               94 &            95 &                    18 &  783 \\
 college\_medicine                    &               77 &            80 &                    15 &  173 \\
 high\_school\_biology                 &               93 &            94 &                    17 &  310 \\
 high\_school\_statistics              &               80 &            85 &                    25 &  216 \\
 high\_school\_psychology              &               93 &            94 &                    18 &  545 \\
 high\_school\_microeconomics          &               90 &            93 &                    29 &  238 \\
 professional\_psychology             &               87 &            86 &                    -5 &  612 \\
 sociology                           &               93 &            91 &                   -27 &  201 \\
 prehistory                          &               92 &            91 &                   -20 &  324 \\
 international\_law                   &               92 &            92 &                     0 &  121 \\
 security\_studies                    &               81 &            82 &                     4 &  245 \\
 electrical\_engineering              &               77 &            81 &                    18 &  145 \\
 management                          &               88 &            90 &                    17 &  103 \\
 human\_sexuality                     &               89 &            89 &                     7 &  131 \\
 logical\_fallacies                   &               85 &            87 &                    12 &  163 \\
 econometrics                        &               73 &            74 &                     3 &  114 \\
 nutrition                           &               87 &            89 &                    15 &  306 \\
 human\_aging                         &               83 &            84 &                     5 &  223 \\
 medical\_genetics                    &               93 &            97 &                    57 &  100 \\
 high\_school\_chemistry               &               74 &            86 &                    47 &  203 \\
 moral\_disputes                      &               82 &            82 &                    -2 &  346 \\
 us\_foreign\_policy                   &               92 &            94 &                    25 &  100 \\
 philosophy                          &               85 &            85 &                    -2 &  311 \\
 global\_facts                        &               63 &            68 &                    14 &  100 \\
 astronomy                           &               89 &            92 &                    29 &  152 \\
 virology                            &               58 &            56 &                    -4 &  166 \\
 college\_biology                     &               97 &            96 &                   -20 &  144 \\
 high\_school\_geography               &               91 &            93 &                    24 &  198 \\
 professional\_medicine               &               91 &            90 &                    -8 &  272 \\
 elementary\_mathematics              &               82 &            95 &                    70 &  378 \\
 high\_school\_physics                 &               72 &            83 &                    42 &  151 \\
 high\_school\_mathematics             &               61 &            82 &                    54 &  270 \\
 anatomy                             &               83 &            82 &                    -4 &  135 \\
 high\_school\_european\_history        &               86 &            85 &                    -9 &  165 \\
 computer\_security                   &               87 &            86 &                    -8 &  100 \\
 high\_school\_government\_and\_politics &               97 &            97 &                   -20 &  193 \\
 world\_religions                     &               91 &            91 &                     0 &  171 \\
 clinical\_knowledge                  &               86 &            87 &                     6 &  265 \\
 abstract\_algebra                    &               71 &            76 &                    17 &  100 \\
 high\_school\_computer\_science        &               92 &            95 &                    37 &  100 \\
 conceptual\_physics                  &               83 &            87 &                    25 &  235 \\
 professional\_accounting             &               69 &            81 &                    39 &  282 \\
 formal\_logic                        &               67 &            74 &                    21 &  126 \\
 high\_school\_world\_history           &               93 &            92 &                   -25 &  237 \\
 machine\_learning                    &               74 &            79 &                    17 &  112 \\
 high\_school\_us\_history              &               94 &            93 &                   -25 &  204 \\
 jurisprudence                       &               88 &            87 &                    -8 &  108 \\
 college\_physics                     &               61 &            80 &                    50 &  102 \\
 college\_chemistry                   &               61 &            65 &                    10 &  100 \\
 public\_relations                    &               75 &            75 &                    -4 &  110 \\
\bottomrule
\end{tabular}}
\end{scriptsize}
\end{table}

\begin{table}[ht]
\centering
\begin{scriptsize}  % Reduced font size
\setlength{\tabcolsep}{4pt}  % Adjust column separation
%\resizebox{\textwidth}{!}{  % Resize to fit within text width
\begin{tabular}{lrrrr}    
\toprule
\multicolumn{5}{c}{CoT - Direct Performance of Meta-Llama 3.1 70b on MMLU Pro Categories}\\
\midrule
Subject          &   Direct Acc (\%) &   CoT Acc (\%) &   Error Reduction (\%) &    N \\
\midrule
 engineering      &               43 &            46 &                     7 &  969 \\
 health           &               66 &            70 &                    11 &  818 \\
 computer science &               60 &            68 &                    22 &  410 \\
 biology          &               73 &            74 &                     7 &  717 \\
 psychology       &               78 &            76 &                   -10 &  798 \\
 math             &               44 &            68 &                    43 & 1351 \\
 business         &               44 &            68 &                    43 &  789 \\
 economics        &               71 &            76 &                    16 &  844 \\
 chemistry        &               40 &            64 &                    40 & 1132 \\
 law              &               49 &            46 &                    -7 & 1101 \\
 physics          &               45 &            66 &                    38 & 1299 \\
 other            &               62 &            68 &                    17 &  924 \\
 history          &               68 &            64 &                   -13 &  381 \\
 philosophy       &               61 &            61 &                    -2 &  499 \\
\bottomrule
\end{tabular}
\end{scriptsize}
\label{tab:all_mmlu_and_mmlupro_slices}
\caption{CoT vs. Direct performances for all categories of MMLU and MMLU Pro for the Llama 3.1 8B and 70B Instruct models.}
\end{table}
